Technical notes: Syntax-aware Representation Learning With Pointer Networks

This is a work-in-progress report, which aims to share preliminary results of a novel sequence-to-sequence schema for dependency parsing that relies on a combination of a BiLSTM and two Pointer Networks (Vinyals et al., 2015), in which the final softmax function has been replaced with the logistic regression. The two pointer networks co-operate to develop a latent syntactic knowledge, by learning the lexical properties of "selection" and the lexical properties of "selectability", respectively. At the moment and without fine-tuning, the parser implementation gets a UAS of 93.14% on the English Penn-treebank (Marcus et al., 1993) annotated with Stanford Dependencies: 2-3% under the SOTA but yet attractive as a baseline of the approach.

==> references.tex <==

\bibliographystyle{acl}
\begin{thebibliography}{}

\bibitem[\protect\citename{Goldberg}2017]{goldberg-methods}
Yoav Goldberg.
\newblock 2017.
\newblock Neural network methods for natural language processing.
\newblock Synthesis Lectures on Human Language Technologies, 10(1):1–309, 2017..

\bibitem[\protect\citename{K{\"{u}}bler \bgroup et al.\egroup
  }2009]{kubler2008dependency}
Sandra K{\"{u}}bler, Ryan~T. McDonald, and Joakim Nivre.
\newblock 2009.
\newblock {\em Dependency Parsing}.
\newblock Synthesis Lectures on Human Language Technologies. Morgan {\&}
  Claypool Publishers.
  
\bibitem[\protect\citename{Chen and Manning}2014]{chen2014fast}
Danqi Chen and Christopher Manning.
\newblock 2014.
\newblock A fast and accurate dependency parser using neural networks.
\newblock In {\em Proceedings of the 2014 Conference on Empirical Methods in
  Natural Language Processing (EMNLP)}, pages 740--750, Doha, Qatar, October.
  Association for Computational Linguistics.

\bibitem[\protect\citename{Dyer \bgroup et al.\egroup
  }2015]{dyer2015transitionbased}
Chris Dyer, Miguel Ballesteros, Wang Ling, Austin Matthews, and Noah~A. Smith.
\newblock 2015.
\newblock Transition-based dependency parsing with stack long short-term
  memory.
\newblock In {\em Proceedings of the 53rd Annual Meeting of the Association for
  Computational Linguistics and the 7th International Joint Conference on
  Natural Language Processing (Volume 1: Long Papers)}, pages 334--343,
  Beijing, China, July. Association for Computational Linguistics.
  
\bibitem[\protect\citename{Kiperwasser and Goldberg}2016]{kiperwasser2016ef}
Eliyahu Kiperwasser and Yoav Goldberg.
\newblock 2016.
\newblock Easy-first dependency parsing with hierarchical tree {LSTMs}.
\newblock {\em Transactions of the Association for Computational Linguistics},
  4.

\bibitem[\protect\citename{Dozat and Manning}2017]{dozat2016deep}
Timothy Dozat and Christopher~D. Manning. 2017.
\newblock 2017.
\newblock Deep biaffine attention for neural dependency parsing.
\newblock In {\em Proc. of ICLR\/}.

\bibitem[\protect\citename{Ballesteros \bgroup et al.\egroup
  }2016]{ballesteros2016dynamic}
Miguel Ballesteros, Yoav Goldberg, Chris Dyer, and Noah~A. Smith.
\newblock 2016.
\newblock Training with exploration improves a greedy stack-{LSTM} parser.
\newblock {\em CoRR}, abs/1603.03793.

\bibitem[\protect\citename{Liu and Zhang}2017]{liu2017encoder}
Jiangming Liu and Yue Zhang
\newblock 2017.
\newblock Encoder-Decoder Shift-Reduce Syntactic Parsing.
\newblock {\em IWPT}, 105-114

\bibitem[\protect\citename{Hochreiter and Schmidhuber}1997]{hochreiter1997long}
Sepp Hochreiter and J{\"{u}}rgen Schmidhuber.
\newblock 1997.
\newblock Long short-term memory.
\newblock {\em Neural Computation}, 9(8):1735--1780.

\bibitem[\protect\citename{Caruana}1997]{Caruana:1997:ML:262868.262872}
Rich Caruana.
\newblock 1997.
\newblock Multitask learning.
\newblock {\em Machine Learning}, 28:41--75, July.

\bibitem[\protect\citename{McDonald \bgroup et al.\egroup }2005]{mst}
Ryan McDonald, Koby Crammer, and Fernando Pereira.
\newblock 2005.
\newblock Online large-margin training of dependency parsers.
\newblock In {\em Proceedings of the 43rd Annual Meeting of the Association for
  Computational Linguistics (ACL'05)}, pages 91--98, Ann Arbor, Michigan, June.
  Association for Computational Linguistics.
  
\bibitem[\protect\citename{Tesni{\`e}re}1959]{Tesniere:1959}
Lucien Tesni{\`e}re.
\newblock 1959.
\newblock {\em El{\'e}ments de Syntaxe Structurale}.
\newblock Klincksieck, Paris.

\bibitem[\protect\citename{Sgall \bgroup et al.\egroup }1986]{Sgall:1986}
Petr Sgall, Eva Haji{\v{c}}ov{\'a}, and Jarmilla Panevov{\'a}.
\newblock 1986.
\newblock {\em The Meaning of the Sentence in Its Semantic and Pragmatic
  Aspects}.
\newblock Reidel, Dordrecht.

\bibitem[\protect\citename{Mel'cuk}1988]{Mel'cuk:1988}
Igor'~A. Mel'cuk.
\newblock 1988.
\newblock {\em Dependency syntax: theory and practice}.
\newblock State Univ. of New York Pr., Albany, NY.

\bibitem[\protect\citename{Hudson}1990]{hudson90}
R.~Hudson.
\newblock 1990.
\newblock {\em English Word Grammar}.
\newblock Basil Blackwell, Oxford.

\bibitem[\protect\citename{Kingma and Ba}2015]{kingma2014adam}
Diederik~P. Kingma and Jimmy Ba.
\newblock 2015.
\newblock Adam: {A} method for stochastic optimization.
\newblock In {\em Proceedings of the 3rd International Conference for Learning
  Representations}, San Diego, California.

\bibitem[\protect\citename{Marcus \bgroup et al.\egroup }1993]{penntb}
Mitchell~P. Marcus, Beatrice Santorini, and Mary~Ann Marcinkiewicz.
\newblock 1993.
\newblock Building a large annotated corpus of {E}nglish: The {P}enn
  {T}reebank.
\newblock {\em Computational Linguistics}, 19(2):313--330.

\bibitem[\protect\citename{Irsoy and Cardie}2014]{irsoy2014opinion}
Ozan Irsoy and Claire Cardie.
\newblock 2014.
\newblock Opinion mining with deep recurrent neural networks.
\newblock In {\em Proceedings of the 2014 Conference on Empirical Methods in
  Natural Language Processing (EMNLP)}, pages 720--728, Doha, Qatar, October.
  Association for Computational Linguistics.

\bibitem[\protect\citename{Graves}2008]{graves2008supervised}
Alex Graves.
\newblock 2008.
\newblock {\em Supervised sequence labelling with recurrent neural networks}.
\newblock {Ph.D.} thesis, Technical University Munich.

\bibitem[\protect\citename{Zhang \bgroup et al.\egroup }2016]{zhang2016dependency}
Xingxing Zhang, Jianpeng Cheng, Mirella Lapata
\newblock 2016.
\newblock Dependency parsing as head selection
\newblock arXiv preprint arXiv:1606.01280
  
\bibitem[\protect\citename{Kiperwasser and Goldberg}2016]{kiperwasser2016simple}
Eliyahu Kiperwasser and Yoav Goldberg.
\newblock 2016.
\newblock Simple and accurate dependency parsing using bidirectional LSTM feature representations.
\newblock {Transactions of the Association for Computational Linguistics}
\newblock 4:313--327. 

\bibitem[\protect\citename{Iyyer \bgroup et al.\egroup }2015]{iyyer2015deep}
Mohit Iyyer, Varun Manjunatha, Jordan Boyd-Graber, and Hal Daum\'{e}~III.
\newblock 2015.
\newblock Deep unordered composition rivals syntactic methods for text
  classification.
\newblock In {\em Proceedings of the 53rd Annual Meeting of the Association for
  Computational Linguistics and the 7th International Joint Conference on
  Natural Language Processing (Volume 1: Long Papers)}, pages 1681--1691,
  Beijing, China, July. Association for Computational Linguistics.

\bibitem[\protect\citename{Zhang and Nivre}2011]{zhang11acl}
Yue Zhang and Joakim Nivre.
\newblock 2011.
\newblock Transition-based dependency parsing with rich non-local features.
\newblock In {\em Proceedings of the 49th Annual Meeting of the Association for
  Computational Linguistics: Human Language Technologies}, pages 188--193,
  Portland, Oregon, USA, June. Association for Computational Linguistics.

\bibitem[\protect\citename{Karpathy \bgroup et al.\egroup
  }2015]{karpathy2015visualizing}
Andrej Karpathy, Justin Johnson, and Fei{-}Fei Li.
\newblock 2015.
\newblock Visualizing and understanding recurrent networks.
\newblock {\em CoRR}, abs/1506.02078.

\bibitem[\protect\citename{Hwa \bgroup et al.\egroup
  }2005]{hwa2005bootstrapping}
Rebecca Hwa, Philip Resnik, Amy Weinberg, Clara Cabezas, Okan Kolak
\newblock 2015.
\newblock Bootstrapping parsers via syntactic projection across parallel texts.
\newblock In {\em Natural language engineering of Cambridge University Press}, 1:3:311--325

\bibitem[\protect\citename{Rumelhart \bgroup et al.\egroup
  }1985]{rumelhart1985learning}
Rumelhart, David E and Hinton, Geoffrey E and Williams, Ronald J
\newblock 1985.
\newblock Learning internal representations by error propagation.
\newblock California Univ San Diego La Jolla Inst for Cognitive Science

\bibitem[\protect\citename{Kenton \bgroup et al.\egroup
  }2017]{lee2017recurrent}
Kenton Lee, Omer Levy, Luke Zettlemoyer
\newblock 2015.
\newblock Visualizing and understanding recurrent networks.
\newblock arXiv preprint arXiv:1705.07393

\bibitem[\protect\citename{Bahdanau \bgroup et al.\egroup
  }2017]{bahdanau2014neural}
Dzmitry Bahdanau, Kyunghyun Cho, Yoshua Bengio
\newblock 2014.
\newblock Neural machine translation by jointly learning to align and translate.
\newblock arXiv preprint arXiv:1409.0473

\bibitem[\protect\citename{Shi \bgroup et al.\egroup
  }2017]{shi2017fast}
Tianze Shi, Liang Huang, Lillian Lee
\newblock 2017.
\newblock Fast(er) Exact Decoding and Global Training for Transition-Based Dependency Parsing via a Minimal Feature Set.
\newblock arXiv preprint arXiv:1708.09403

\bibitem[\protect\citename{Bengio \bgroup et al.\egroup
  }2003]{bengio2003neural}
Yoshua Bengio, Réjean Ducharme, Pascal Vincent, Christian Jauvin
\newblock 2003.
\newblock A neural probabilistic language model.
\newblock In {\em Journal of machine learning research} 3:1137--1155

\bibitem[\protect\citename{Jiang \bgroup et al.\egroup
  }2016]{jiang2016unsupervised}
Yoshua Bengio, Réjean Ducharme, Pascal Vincent, Christian Jauvin
\newblock 2016.
\newblock Unsupervised neural dependency parsing.
\newblock In {\em Proceedings of the 2016 Conference on Empirical Methods in Natural Language Processing}, pages 763--771

\bibitem[\protect\citename{Frazier and Rayner
  }1982]{frazier1982making}
Lyn Frazier and Keith Rayner.
\newblock 1982.
\newblock Making and correcting errors during sentence comprehension: Eye movements in the analysis of structurally ambiguous sentences.
\newblock Elsevier, Cognitive psychology 14:2:178--210

\bibitem[\protect\citename{Rama \bgroup et al.\egroup
  }2016]{rama2016lstm}
Rama, Taraka and {\c{C}}{\"o}ltekin, {\c{C}}a{\u{g}}r{\i}
\newblock 2016.
\newblock LSTM autoencoders for dialect analysis.
\newblock In {\em Proceedings of the Third Workshop on NLP for Similar Languages, Varieties and Dialects (VarDial3)}, pages 25--32

\bibitem[\protect\citename{Grella}2018]{grella2018taking}
Matteo Grella
\newblock 2018.
\newblock Taking Advantage of BiLSTM Encoding to Handle Punctuation in Dependency Parsing: A Brief Idea

\bibitem[\protect\citename{Ficler and Yoav}2017]{ficler2017improving}
Jessica Ficler and Yoav Goldberg
\newblock 2017.
\newblock Improving a Strong Neural Parser with Conjunction-Specific Feature.
\newblock arXiv preprint arXiv:1702.06733

\bibitem[\protect\citename{Dozat \bgroup et al.\egroup
  }2017]{dozat2017stanford}
Dozat, Timothy and Qi, Peng and Manning, Christopher D
\newblock 2017.
\newblock Stanford's Graph-based Neural Dependency Parser at the CoNLL 2017 Shared Task
\newblock In {\em Proceedings of the CoNLL 2017 Shared Task: Multilingual Parsing from Raw Text to Universal Dependencies}, pages 20--30

\bibitem[\protect\citename{Grella}2017]{11372/LRT-2288}
Matteo Grella
\newblock 2017.
\newblock Italian Function Words
\newblock http://hdl.handle.net/11372/LRT-2288
\newblock {LINDAT}/{CLARIN} digital library at the Institute of Formal and Applied Linguistics ({{\\'U}FAL}), Faculty of Mathematics and Physics, Charles University

\bibitem[\protect\citename{Grella}2017]{11372/LRT-2476}
Matteo Grella
\newblock 2017.
\newblock Italian Content Words
\newblock http://hdl.handle.net/11372/LRT-2476
\newblock {LINDAT}/{CLARIN} digital library at the Institute of Formal and Applied Linguistics ({{\\'U}FAL}), Faculty of Mathematics and Physics, Charles University

\end{thebibliography}

